Stable high-dimensional weak-light soliton molecules and their active control

Bound states of solitons, alias soliton molecules (SMs), are well known in one-dimensional (1D) systems, while making stable bound states of multidimensional solitons is a challenging problem because of the underlying instabilities. Here we propose a scheme for the creation of stable (2+1)D and (3+1)D optical SMs in a gas of cold Rydberg atoms, in which electromagnetically induced transparency (EIT) is induced by a control laser field. We show that, through the interplay of the EIT and the strong long-range interaction between the Rydberg atoms, the system gives rise to giant nonlocal Kerr nonlinearity, which in turn supports stable (2+1)D spatial optical SMs, as well as ring-shaped soliton necklaces, including rotating ones. They feature a large size, low generation power, and can be efficiently manipulated by tuning the nonlocality degree of the Kerr nonlinearity. Stable (3+1)D spatiotemporal optical SMs, composed of fundamental or vortex solitons, with low power and ultraslow propagation velocity, can also be generated in the system. These SMs can be stored and retrieved through the switching off and on of the control laser field. The findings reported here suggest applications to data processing and transmission in optical systems.

==> references <==
@article{kuznetsov1986soliton,
  title={Soliton stability in plasmas and hydrodynamics},
  author={Kuznetsov, EA and Rubenchik, AM and Zakharov, Vladimir E},
  journal={Physics Reports},
  volume={142},
  number={3},
  pages={103--165},
  year={1986},
  publisher={Elsevier}
}



@article{ Rubenchik,
title ={Soliton stability in plasmas and hydrodynamics},
author ={  E. A. Kuznetsov and },
journal ={ '' Phys. Rep. },
volume = {142},
pages = { 103--165 },
year = {1986}
}

@article{ Lederer,
title ={Discrete solitons in optics},
author ={  F. Lederer and  G. I. Stegemanand  D. N. Christodoulidesand  G. Assantoand  M. Segev},
journal ={ " Phys. Rep. },
volume = {463},
pages = { 1--126 },
year = {2008}
}

@article{ Wadati,
title ={Soliton propagations in the electromagnetically induced transparency},
author ={  M. Wadati and },
journal ={ " Eur. Phys. J. Spec. Top. },
volume = {173},
pages = { 223--232 },
year = {2009}
}

@article{ Maimistov,
title ={Solitons in nonlinear optics},
author ={  A. I. Maimistov and },
journal ={ " Quantum Electron. },
volume = {40},
pages = { 756--781 },
year = {2010}
}

@article{ Turitsyn,
title ={Dispersion-managed solitons in fibre systems and lasers},
author ={  S. K. Turitsyn and  B. G. Bale},
journal ={ " Phys. Rep. },
volume = {521},
pages = { 135--203 },
year = {2012}
}

@article{ Grelu2012,
title ={Dissipative solitons for mode-locked lasers},
author ={  P. Grelu and N. Akhmediev and },
journal ={ " Nat. Photon. },
volume = {6},
pages = { 84--92 },
year = {2012}
}


@article{ Konotop,
title ={Theory of nonlinear matter waves in optical lattices"},
author ={  V. A. Brazhnyi and V. V. Konotop and },
journal ={  Mod. Phys. Lett. },
volume = {18},
pages = { 627--651 },
year = {2004}
}

@article{ Abdullaev,
title ={Dynamics of bright matter wave solitons in a Bose Einstein condensate"},
author ={  F. Kh. Abdullaev and  A. Gammaland  A. M. Kamchatnov},
journal ={  Int. J. Mod. Phys. B },
volume = {19},
pages = { 3415--3473 },
year = {2005}
}

@article{ DFrantz,
title ={Dark solitons in atomic Bose-Einstein condensates: from theory to experiments"},
author ={  D. J. Frantzeskakis and },
journal ={  J. Phys. A: Math. Theor. },
volume = {43},
pages = { 213001 },
year = {2010}
}

@article{ Salasnich,
title ={Bright solitons in ultracold atoms},
author ={  L. Salasnich and },
journal ={ " Opt. Quant. Electron. },
volume = {49},
pages = { 409 },
year = {2017}
}

@article{ Barcelona,
title ={Solitons in nonlinear lattices},
author ={  Y. V. Kartashov and  B. A. Malomed},
journal ={ '' Rev. Mod. Phys. },
volume = {83},
pages = { 247--305 },
year = {2011}
}

@article{ Tappert1971,
title ={Gradient-Induced Fission of Solitons},
author ={  F. D. Tappert and N. J. Zabusky and },
journal ={ '' Phys. Rev. Lett. },
volume = {27},
pages = { 1774 },
year = {1971}
}

@article{ RMP,
title ={Dynamics of solitons in nearly integrable systems},
author ={  Y. S. Kivshar and B. A. Malomed and },
journal ={ '' Rev. Mod. Phys. },
volume = {61},
pages = { 763-915 },
year = {1989}
}

@article{ Tikhonenko1996,
title ={Three Dimensional Bright Spatial Soliton Collision and Fusion in a Saturable Nonlinear Medium},
author ={  V. Tikhonenko and  J. Christou},
journal ={ '' Phys. Rev. Lett. },
volume = {76},
pages = { 2698 },
year = {1996}
}

@article{ Krolikowski1997,
title ={Fusion and birth of spatial solitons upon collision},
author ={  W. Krolikowski and S. A. Holmstrom and },
journal ={ '' Opt. Lett. },
volume = {22},
pages = { 369--371 },
year = {1997}
}

@article{ Krolikowski1998,
title ={Annihilation of photorefractive solitons},
author ={  W. Krolikowski and  B. Luther-Daviesand  C. Denz},
journal ={ '' Opt. Lett. },
volume = {23},
pages = { 97--99 },
year = {1998}
}

@article{ Herrmann,
title ={Soliton collision and soliton fusion in dispersive linear materials with a linear and quadratic intensity depending refraction index change},
author ={  S. Gatz and J. Herrmann and },
journal ={ '' IEEE J. Quantum Electron },
volume = {28},
pages = { 1732--1738 },
year = {1992}
}

@article{ Lu2004,
title ={Vector Soliton Fission},
author ={  F. Lu and  Q. Linand  W. H. Knox},
journal ={ '' Phys. Rev. Lett. },
volume = {93},
pages = { 183901 },
year = {2004}
}

@article{ Pfeiffer2006,
title ={Observation of Soliton Fusion in a Josephson Array},
author ={  J. Pfeiffer and  M. Schusterand  A. A. Abdumalikovand  Jr.},
journal ={ '' Phys. Rev. Lett. },
volume = {96},
pages = { 034103 },
year = {2006}
}

@article{ Randy,
title ={Collisions of matter-wave solitons},
author ={  J. H. V. Nguyen and  P. Dykeand  D. Luoand  B. A. Malomed},
journal ={ '' Nat. Phys. },
volume = {10},
pages = { 918--922 },
year = {2014}
}

@article{ Descalzi2009,
title ={Noise Induces Partial Annihilation of Colliding Dissipative Solitons},
author ={  O. Descalzi and  J. Cisternasand  D. Escaff},
journal ={ '' Phys. Rev. Lett. },
volume = {102},
pages = { 188302 },
year = {2009}
}

@article{ Maiden2014,
title ={d annihilation in magnetic droplet soliton scattering},
author ={  M. D. Maiden and  L. D. Bookmanand  and M. A. Hoeferand  ``Attractionand  merger},
journal ={ '' Phys. Rev. B },
volume = {89},
pages = { 180409},
year = {R}
}

@article{ Kottig2017,
title ={PHz-Wide Spectral Interference Through Coherent Plasma-Induced Fission of Higher Order Solitons},
author ={  F. K\"ottig and  F. Taniand  J. C. Travers},
journal ={ '' Phys. Rev. Lett. },
volume = {118},
pages = { 263902 },
year = {2017}
}

@article{ Descalzi2020,
title ={Breaking of symmetry of interacting dissipative solitons can lead to partial annihilation},
author ={  O. Descalzi and H. R. Brand and },
journal ={ '' Phys. Rev. E },
volume = {101},
pages = { 040201},
year = {R}
}

@article{ Malomed1991,
title ={Bound solitons in the nonlinear Schr\"{o}dinger-Ginzburg-Landau equation},
author ={  B. A. Malomed and },
journal ={ " Phys. Rev. A },
volume = {44},
pages = { 6954 },
year = {1991}
}

@article{ Malomed1993,
title ={Bound states of envelope solitons},
author ={  B. A. Malomed and },
journal ={ " Phys. Rev. A },
volume = {47},
pages = { 2874 },
year = {1993}
}

@article{ Nepom,
title ={Stability limits for arrays of kinks in two-component nonlinear systems},
author ={  B. A. Malomed and A. A. Nepomnyashchy and },
journal ={ " Europhys. Lett. },
volume = {27},
pages = { 649-653 },
year = {1994}
}

@article{ random,
title ={Bound states in a gas of solitons supported by a randomly fluctuating force},
author ={  B. A. Malomed and },
journal ={ '' Europhys. Lett. },
volume = {30},
pages = { 507--512 },
year = {1995}
}

@article{ Afanasjev1997,
title ={Stability of bound states of pulses in the Ginzburg-Landau equations},
author ={  V. V. Afanasjev and  B. A. Malomed},
journal ={ '' Phys. Rev. E },
volume = {56},
pages = { 6020 },
year = {1997}
}

@article{ Tang-1,
title ={Observation of bound states of solitons in a passively mode-locked fiber laser},
author ={  D. Y. Tang and  W. S. Manand  H. Y. Tam},
journal ={ '' Phys. Rev. A },
volume = {64},
pages = { 033814 },
year = {2001}
}

@article{ Tang-2,
title ={Soliton interaction in a fiber ring laser},
author ={  D. Y. Tang and  B. Zhaoand  L. M. Zhao},
journal ={ '' Phys. Rev. E },
volume = {72},
pages = { 016616 },
year = {2005}
}

@article{ Komarov2009,
title ={Quantization of binding energy of structural solitons in passive mode-locked fiber lasers},
author ={  A. Komarov and  K. Komarov},
journal ={ '' Phys. Rev. A },
volume = {79},
pages = { 033807 },
year = {2009}
}

@article{ Wang2017,
title ={Universal mechanism for the binding of temporal cavity solitons},
author ={  Y. Wang and  F. Leoand  J. Fatomeand  M. Erkintaloand  S. G. Murdoch},
journal ={ '' Optica },
volume = {4},
pages = { 855--863 },
year = {2017}
}

@article{ Skryabin,
title ={Stationary and oscillatory bound states of dissipative solitons created by the third-order dispersion},
author ={  H. Sakaguchi and  D. V. Skryabin},
journal ={ '' Opt. Lett. },
volume = {43},
pages = { 2688--2691 },
year = {2018}
}

@article{ Gelash2019,
title ={Bound State Soliton Gas Dynamics Underlying the Spontaneous Modulational Instability},
author ={  A. Gelash and  D. Agafontsevand  V. Zakharovand  G. Eland  S. Randoux},
journal ={ '' Phys. Rev. Lett. },
volume = {123},
pages = { 234102 },
year = {2019}
}

@article{ Akhmediev1997,
title ={Multisoliton Solution of the Complex Ginzburg-Landau Equation},
author ={  N. N. Akhmediev and A. Ankiewicz and },
journal ={ '' Phys. Rev. Lett. },
volume = {79},
pages = { 4047 },
year = {1998}
}

@article{ Crasovan2003,
title ={Soliton `molecules': Robust clusters of spatiotemporal optical solitons},
author ={  L.-C. Crasovan and  Y. V. Kartashovand  D. Mihalacheand  L. Tornerand  Y. S. Kivshar},
journal ={ '' Phys. Rev. E },
volume = {67},
pages = { 046610 },
year = {2003}
}

@article{ Vekslerchik2003,
title ={Soliton molecules in trapped vector nonlinear Schr\"odinger systems},
author ={  V. M. P\' and },
journal ={ '' Phys. Rev. E },
volume = {67},
pages = { 061804 },
year = {2003}
}

@article{ Stratmann2005,
title ={Experimental Observation of Temporal Soliton Molecules},
author ={  M. Stratmann and  T. Pagel},
journal ={ '' Phys. Rev. Lett. },
volume = {95},
pages = { 143902 },
year = {2005}
}

@article{ Hause2008,
title ={Binding mechanism of temporal soliton molecules},
author ={  A. Hause and  H. Hartwigand  M. B\"{o}hm},
journal ={ '' Phys. Rev. A },
volume = {78},
pages = { 063817 },
year = {2008}
}

@article{ Leblond,
title ={Coherent soliton pattern formation in a fiber laser},
author ={  A. Haboucha and  H. Leblondand  M. Salhiand  A. Komarov},
journal ={ '' Opt. Lett. },
volume = {33},
pages = { 524--526 },
year = {2008}
}

@article{ Zavyalov2009,
title ={Dissipative soliton molecules with independently evolving or flipping phases in mode-locked fiber lasers},
author ={  A. Zavyalov and  R. Iliewand  O. Egorov},
journal ={ '' Phys. Rev. A },
volume = {80},
pages = { 043829 },
year = {2009}
}

@article{ Khawaja2010,
title ={Stability and dynamics of two-soliton molecules},
author ={  U. Al Khawaja and },
journal ={ '' Phys. Rev. E },
volume = {81},
pages = { 056603 },
year = {2010}
}


@article{ Khawaja2011,
title ={Formation of matter-wave soliton molecules},
author ={  U. Al Khawaja and H. T. C. Stoof and },
journal ={ '' New J. Phys. },
volume = {13},
pages = { 085003 },
year = {2011}
}

@article{ Santos2012,
title ={Soliton molecules in dipolar Bose-Einstein condensates},
author ={  K. Lakomy and  R. Nath},
journal ={ '' Phys. Rev. A },
volume = {86},
pages = { 013610 },
year = {2012}
}

@article{ Rohrmann2013,
title ={Two-soliton and three-soliton molecules in optical fibers},
author ={  P. Rohrmann and  A. Hause},
journal ={ '' Phys. Rev. A },
volume = {87},
pages = { 043834 },
year = {2013}
}

@article{ Boudje2013,
title ={Stability of N-soliton molecules in dispersion-managed optical fibers},
author ={  A. Boudjem\^ and },
journal ={ '' Phys. Rev. A },
volume = {88},
pages = { 045801 },
year = {2013}
}

@article{ Hause2013,
title ={Higher-order equilibria of temporal soliton molecules in dispersion-managed fibers},
author ={  A. Hause and F. Mitschke and },
journal ={ '' Phys. Rev. A },
volume = {88},
pages = { 063843 },
year = {2013}
}

@article{ Shirley2014,
title ={Half-Quantum Vortex Molecules in a Binary Dipolar Bose Gas},
author ={  W. E. Shirley and  B. M. Andersonand  C. W. Clark},
journal ={ '' Phys. Rev. Lett },
volume = {113},
pages = { 165301 },
year = {2014}
}

@article{ Alamoudi2014,
title ={Averaged dynamics of soliton molecules in dispersion-managed optical fibers},
author ={  S. M. Alamoudi and  U. Al Khawaja},
journal ={ '' Phys. Rev. A },
volume = {89},
pages = { 053817 },
year = {2014}
}

@article{ Turmanov2015,
title ={Vibration spectrum of a two-soliton molecule in dipolar Bose-Einstein condensates},
author ={  B. K. Turmanov and  B. B. Baizakovand  B. A. Umarov},
journal ={ '' Phys. Lett. A },
volume = {379},
pages = { 1828--1832 },
year = {2015}
}

@article{ Baizakov2015,
title ={Interaction of soliton in one-dimensional dipolar Bose-Einstein condensates and formation of soliton molecules},
author ={  B. B. Baizakov and  S. M. Al-Marzoug},
journal ={ '' Phys. Rev. A },
volume = {92},
pages = { 033605 },
year = {2015}
}

@article{ Leblond-2,
title ={Influence of gain dynamics on dissipative soliton interaction in the presence of a continuous wave},
author ={  A. Niang and  F. Amraniand  M. Salhiand  H. Leblond},
journal ={ '' Phys. Rev. A },
volume = {92},
pages = { 033831 },
year = {2015}
}

@article{ Wang2016,
title ={Generation of wavelength-tunable soliton molecules in a 2-$ \mu\mathrm{m}$ ultrafast all-fiber laser based on nonlinear polarization evolution},
author ={  P. Wang and  C. Baoand  B. Fuand  X. Xiaoand  P. Grelu},
journal ={ " Opt. Lett. },
volume = {41},
pages = { 2254--2257 },
year = {2016}
}

@article{ Herink2017,
title ={d C. Ropers ``Real-time spectral interferometry probes the internal dynamics of femtosecond soliton molecules},
author ={  G. Herink and  F. Kurtz},
journal ={ '' Science },
volume = {356},
pages = { 50--54 },
year = {2017}
}

@article{ Krupa2017,
title ={Real-Time Observation of Internal Motion within Ultrafast Dissipative Optical Soliton Molecules},
author ={  K. Krupa and  K. Nithyanandanand  U. Andraland  P. Tchofo-Dinda},
journal ={ '' Phys. Rev. Lett. },
volume = {118},
pages = { 243901 },
year = {2017}
}

@article{ YiyangLuo2017,
title ={Group-velocity-locked vector soliton molecules in fiber lasers},
author ={  Y. Luo and  J. Chengand  B. Liuand  Q. Sunand  L. Liand  S. Fuand  D. Tangand  L. Zhao},
journal ={ '' Sci. Rep. },
volume = {7},
pages = { 2369 },
year = {2017}
}

@article{ XuemingLiu2018,
title ={Real-Time Observation of Buildup of Soliton Molecules},
author ={  X. Liu and  X. Yao},
journal ={ '' Phys. Rev. Lett },
volume = {121},
pages = { 023905 },
year = {2018}
}

@article{ Qin2018,
title ={Observation of soliton molecules in a spatiotemporal mode-locked multimode fiber laser},
author ={  H. Qin and  X. Xiaoand  P. Wang},
journal ={ '' Opt. Lett. },
volume = {43},
pages = { 1982--1985 },
year = {2018}
}

@article{ JunsongPeng2018,
title ={Bulid-Up of Dissipative Optical Soliton Molecules via Diverse Soliton Interaction},
author ={  J. Peng and H. Zeng and },
journal ={ '' Laser Photon. Rev. },
volume = {12},
pages = { 1800009 },
year = {2018}
}

@article{ GangXu2019,
title ={Breather Wave Molecules},
author ={  G. Xu and  A. Gelashand  A. Chabchouband  V. Zakharov},
journal ={ '' Phys. Rev. Lett. },
volume = {122},
pages = { 084101 },
year = {2019}
}

@article{ Melchert2019,
title ={Soliton Molecules with Two Frequencies},
author ={  O. Melchert and  S. Willmsand  S. Boseand  A. Yulinand  B. Rothand  F. Mitschkeand  U. Morgnerand  I. Babushkin},
journal ={ '' Phys. Rev. Lett. },
volume = {123},
pages = { 243905 },
year = {2019}
}

@article{ Wang2019,
title ={Optical soliton molecular complexes in a passively mode-locked fibre laser},
author ={  Z. Q. Wang and  K. Nithyanandanand  A. Coilletand  P. Tchofo-Dinda},
journal ={ '' Nat. Commun. },
volume = {10},
pages = { 830 },
year = {2019}
}

@article{ ZhouY2020,
title ={Buildup and dissociation dynamics of dissipative optical soliton molecules},
author ={  Y. Zhou and  Y.-X. Renand  J. Shiand  H. Mao},
journal ={ '' Optica },
volume = {7},
pages = { 965--972 },
year = {2020}
}

@article{ Kurtz2020,
title ={Resonant excitation and all-optical switching of femtosecond soliton molecules},
author ={  F. Kurtz and  C. Ropers},
journal ={ '' Nat. Photon. },
volume = {14},
pages = { 9--13 },
year = {2020}
}

@article{ Weng2020,
title ={Heteronuclear soliton molecules in optical microresonators},
author ={  W. Weng and  R. Bouchandand  E. Lucasand  E. Obrzudand  T. Herr},
journal ={ " Nat. Commun. },
volume = {11},
pages = { 2402 },
year = {2020}
}

@article{ Maitre2020,
title ={Dark-Soliton Molecules in an Exciton-Polariton Superfluid},
author ={  A. Ma\^ and  G. Lerarioand  A. Medeirosand  F. Claudeand  Q. Glorieuxand  E. Giacobinoand  S. Pigeon},
journal ={ '' Phys. Rev. X },
volume = {10},
pages = { 041028 },
year = {2020}
}

@article{ Berge',
title ={Wave collapse in physics: principles and applications to light and plasma waves},
author ={  L. Berg\' and },
journal ={ '' Phys. Rep. },
volume = {303},
pages = { 259--370 },
year = {1998}
}

@article{ spatiotemp,
title ={Spatiotemporal optical solitons},
author ={  B. A. Malomed and  D. Mihalacheand  F. Wise},
journal ={ '' J. Optics B: Quant. Semicl. Opt. },
volume = {7},
pages = { R53--R72 },
year = {2005}
}

@article{ Michinel,
title ={Stable azimuthal stationary state in quintic nonlinear optical media},
author ={  M. Quiroga-Teixeiro and H. Michinel and },
journal ={ '' J. Opt. Soc. Am. B },
volume = {14},
pages = { 2004--2009 },
year = {1997}
}

@article{ Pego,
title ={Spectrally stable encapsulated vortices for nonlinear Schr\"{o}dinger equations},
author ={  R. L. Pego and H. A. Warchall and },
journal ={ '' J. Nonlinear Sci. },
volume = {12},
pages = { 347--394 },
year = {2002}
}

@article{ vortices,
title ={(INVITED)\ Vortex solitons: Old results and new perspectives},
author ={  B. A. Malomed and },
journal ={ " Physica D },
volume = {399},
pages = { 108--137 },
year = {2019}
}

@article{ Special topics,
title ={Multidimensional solitons: Well-established results and novel findings},
author ={  B. A. Malomed and },
journal ={ " Eur. Phys. J. Spec. Top. },
volume = {225},
pages = { 2507--2532 },
year = {2016}
}

@article{ Astra,
title ={Frontiers in multidimensional self-trapping of nonlinear fields and matter},
author ={  Y. V. Kartashov and  G. E. Astrakharchikand  B. A. Malomed},
journal ={ " Nat. Rev. Phys. },
volume = {1},
pages = { 185--197 },
year = {2019}
}

@article{ Kengne,
title ={Spatiotemporal engineering of matter-wave solitons in Bose-Einstein condensates},
author ={  E. Kengne and  W.-M. Liu},
journal ={ " Phys. Rep. },
volume = {899},
pages = { 1--62 },
year = {2021}
}

@article{ Cid,
title ={Robust two-dimensional spatial solitons in liquid carbon disulfide},
author ={  E. L. Falc\~ and  C. B. de Ara\'{u}joand  G. Boudebsand  H. Leblond},
journal ={ '' Phys. Rev. Lett. },
volume = {110},
pages = { 013901 },
year = {2013}
}

@article{ Leticia,
title ={Quantum liquid droplets in a mixture of Bose--Einstein condensates},
author ={  C. R. Cabrera and  L. Tanziand  J. Sanzand  B. Naylorand  P. Thomasand  P. Cheiney},
journal ={ '' Science },
volume = {359},
pages = { 301--304 },
year = {2018}
}

@article{ Leticia2,
title ={Bright soliton to quantum droplet transition in a mixture of Bose--Einstein condensates},
author ={  P. Cheiney and  C. R. Cabreraand  J. Sanzand  B. Naylorand  L. Tanzi},
journal ={ '' Phys. Rev. Lett. },
volume = {120},
pages = { 135301 },
year = {2018}
}

@article{ Inguscio,
title ={Self-bound quantum droplets of atomic mixtures in free space},
author ={  G. Semeghini and  G. Ferioliand  L. Masiand  C. Mazzinghiand  L. Wolswijkand  F. Minardiand  M. Modugnoand  G. Modugnoand  M. Inguscio},
journal ={ '' Phys. Rev. Lett. },
volume = {120},
pages = { 235301 },
year = {2018}
}

@article{ hetero,
title ={Observation of quantum droplets in a heteronuclear bosonic mixture},
author ={  C. D'Errico and  A. Burchiantiand  M. Prevedelliand  L. Salasnichand  F. Ancilottoand  M. Modugnoand  F. Minardi},
journal ={ " Phys. Rev. Research },
volume = {1},
pages = { 033155 },
year = {2019}
}

@article{ Pfau,
title ={New states of matter with fine-tuned interactions: quantum droplets and dipolar supersolids},
author ={  F. B\" and  J.-N. Schmidtand  J. Hertkornand  K. S. H. Ngand  S. D. Grahamand  M. Guoand  T. Langen},
journal ={ " Rep. Prog. Phys. },
volume = {84},
pages = { 012403 },
year = {2020}
}

@article{ droplets,
title ={A new form of liquid matter: quantum droplets},
author ={  Z. Luo and  W. Pangand  B. Liuand  Y. Li},
journal ={ "  Front. Phys. },
volume = {16},
pages = { 32201 },
year = {2021}
}

@article{ Cid2,
title ={Robust self-trapping of vortex beams in a saturable optical medium},
author ={  A. S. Reyna and  G. Boudebsand  B. A. Malomed},
journal ={ '' Phys. Rev. A },
volume = {93},
pages = { 013840 },
year = {2016}
}

@article{ Snyder1997,
title ={Accessible Solitons},
author ={  A. W. Snyder and D. J. Mitchell and },
journal ={ '' Science },
volume = {276},
pages = { 1538--1541 },
year = {1997}
}

@article{ Krolikowski2000,
title ={Solitons in nonlocal nonlinear media: Exact solutions},
author ={  W. Kr\' and },
journal ={ " Phys. Rev. E },
volume = {63},
pages = { 016610 },
year = {2000}
}

@article{ Conti2004,
title ={servation of optical spatial solitons in a highly nonlocal medium},
author ={  C. Conti and  M. Peccianti},
journal ={  Phys. Rev. Lett. },
volume = {92},
pages = { 113902 },
year = {2004}
}

@article{ Xu2005,
title ={Soliton Mobility in Nonlocal Optical Lattices},
author ={  Z. Xu and  Y. V. Kartashov},
journal ={ " Phys. Rev. Lett. },
volume = {95},
pages = { 113901 },
year = {2005}
}

@article{ Alberucci2006,
title ={Two-Color Vector Solitons In Nonlocal Media},
author ={  A. Alberucci and  M. Pecciantiand  G. Assantoand  A. Dyadyusha},
journal ={ '' Phys. Rev. Lett. },
volume = {97},
pages = { 153903 },
year = {2006}
}

@article{ Buccoliero2007,
title ={Laguerre and Hermite Soliton Clusters in Nonlocal Nonlinear Media},
author ={  D. Buccoliero and  A. S. Desyatnikovand  W. Krolikowski},
journal ={ '' Phys. Rev. Lett. },
volume = {98},
pages = { 053901 },
year = {2007}
}

@article{ Skupin2007,
title ={Nonlocal Stabilization of Nonlinear Beams in a Self-Focusing Atomic Vapor},
author ={  S. Skupin and  M. Saffman},
journal ={ '' Phys. Rev. Lett. },
volume = {98},
pages = { 263902 },
year = {2007}
}

@article{ Burgess2009,
title ={Accessible Light Bullets via Synergetic Nonlinearities},
author ={  I. B. Burgess and  M. Pecciantiand  G. Assanto},
journal ={ '' Phys. Rev. Lett. },
volume = {102},
pages = { 203903 },
year = {2009}
}

@article{ Conti2010,
title ={Highly Noninstantaneous Solitons in Liquid-Core Photonic Crystal Fibers},
author ={  C. Conti and  M. A. Schmidtand  P. St. J. Russell},
journal ={ '' Phys. Rev. Lett. },
volume = {105},
pages = { 263902 },
year = {2010}
}

@article{ Sevincli2011,
title ={Nonlocal Nonlinear Optics in Cold Rydberg Gases},
author ={  S. Sevin\c and  N. Henkeland  C. Ates},
journal ={ '' Phys. Rev. Lett. },
volume = {107},
pages = { 153001 },
year = {2011}
}

@article{ Maucher2011,
title ={Rydberg-Induced Solitons: Three-Dimensional Self-Trapping of Matter Waves},
author ={  F. Maucher and  N. Henkeland  M. Saffmanand  W. Kr\'olikowskiand  S. Skupin},
journal ={ '' Phys. Rev. Lett. },
volume = {106},
pages = { 170401 },
year = {2011}
}

@article{ Lahav2017,
title ={Three-Dimensional Spatiotemporal Pulse-Train Solitons},
author ={  O. Lahav and  O. Kfirand  P. Sidorenkoand  M. Mutzafiand  A. Fleischer},
journal ={ '' Phys. Rev. X },
volume = {7},
pages = { 041051 },
year = {2017}
}

@article{ Horikis2017,
title ={Light Meets Water in Nonlocal Media: Surface Tension Analogue in Optics},
author ={  T. P. Horikis and D. J. Frantzeskakis and },
journal ={ '' Phys. Rev. Lett. },
volume = {118},
pages = { 243903 },
year = {2017}
}

@article{ Li2018,
title ={Electrically driven three-dimensional solitary waves as director bullets in nematic liquid crystals},
author ={  B.-X. Li and  V. Borshchand  R.-L. Xiaoand  S. Paladuguand  T. Turivand  S. V. Shiyanovskii},
journal ={ '' Nat. Commun. },
volume = {9},
pages = { 2912 },
year = {2018}
}

@article{ Wilson2018,
title ={Observation of Photon Droplets and Their Dynamics},
author ={  K. E. Wilson and  N. Westerbergand  M. Valienteand  C. W. Duncanand  E. M. Wrightand  P. \"{O}hberg},
journal ={ '' Phys. Rev. Lett. },
volume = {121},
pages = { 133903 },
year = {2018}
}

@article{ Bai2019,
title ={able single light bullets and vortices and their active control in cold Rydberg gases},
author ={  Z. Bai and  W. Li},
journal ={ '' Optica },
volume = {6},
pages = { 309--317 },
year = {2019}
}

@article{ Rotschild2006,
title ={Long-range interactions between optical solitons},
author ={  C. Rotschild and  B. Alfassiand  O. Cohen},
journal ={ '' Nat. Phys. },
volume = {2},
pages = { 769--774 },
year = {2006}
}

@article{ Vardi,
title ={Anisotropic Solitons in Dipolar Bose-Einstein Condensates},
author ={  I. Tikhonenkov and  B. A. Malomed},
journal ={ '' Phys. Rev. Lett. },
volume = {100},
pages = { 090406 },
year = {2008}
}

@article{ Fleischhauer2005,
title ={Electromagnetically induced transparency: optics in coherent media},
author ={  M. Fleischhauer and  A. Imamoglu},
journal ={ '' Rev. Mod. Phys. },
volume = {77},
pages = { 633--673 },
year = {2005}
}

@article{ Saffman2010,
title ={Quantum information with Rydberg atoms},
author ={  M. Saffman and  T. G. Walker},
journal ={ " Rev. Mod. Phys. },
volume = {82},
pages = { 2313--2363 },
year = {2010}
}


@article{ Firstenberg2016,
title ={Nonlinear quantum optics mediated by Rydberg interactions},
author ={  O. Firstenberg and  C. S. Adams},
journal ={ '' J. Phys. B: At. Mol. Opt. Phys. },
volume = {49},
pages = { 152003 },
year = {2016}
}

@article{ Murray2016,
title ={Quantum and nonlinear optics in strongly interacting atomic ensembles},
author ={  C. Murray and T. Pohl and },
journal ={ '' Adv. Mol. Opt. Phys. },
volume = {65},
pages = { 321--372 },
year = {2016}
}

@article{ Bai2016,
title ={Enhanced third-order and fifth-order Kerr nonlinearities in a cold atomic system via atom-atom interaction},
author ={  Z. Bai and G. Huang and },
journal ={ " Opt. Express },
volume = {24},
pages = { 4442--4461 },
year = {2016}
}

@article{ Adams2017,
title ={Contactless nonlinear optics mediated by long-range Rydberg interactions},
author ={  H. Busche and  P. Huilleryand  S. W. Balland  T. Ilievaand  M. P. A. Jones},
journal ={ '' Nat. Phys. },
volume = {13},
pages = { 655--658 },
year = {2017}
}

@article{ Mu2021,
title ={Giant Kerr nonlinearities and magneto-optical rotations in a Rydberg-atom gas via double electromagnetically induced transparency},
author ={  Y. Mu and  L. Qinand  Z. Shi},
journal ={ '' Phys. Rev. A },
volume = {103},
pages = { 043709 },
year = {2021}
}

@article{ potential,
title ={Potential of interaction between two- and three-dimensional solitons},
author ={  B. A. Malomed and },
journal ={ '' Phys. Rev. E },
volume = {58},
pages = { 7928--7933 },
year = {1998}
}

@article{ VA,
title ={Variational methods in nonlinear fiber optics and related fields},
author ={  B. A. Malomed and },
journal ={ '' Prog. Optics },
volume = {43},
pages = { 71--193 },
year = {2002}
}

@article{ Raghavan2000,
title ={Spatiotemporal solitons in inhomogeneous nonlinear media},
author ={  S. Raghavan and G. P. Agrawal and },
journal ={ '' Opt. Commun. },
volume = {180},
pages = { 377--382 },
year = {2000}
}

@article{ Bloch,
title ={Observation of spatially ordered structures in a two-dimensional Rydberg gas},
author ={  P. Schauß and  M. Cheneauand  M. Endresand  T. Fukuharaand  S. Hildand  A. Omranand  T. Pohland  C. Grossand  S. Kuhr},
journal ={ '' Nature },
volume = {491},
pages = { 87--91 },
year = {2012}
}

@article{ necklace,
title ={Laguerre and Hermite Soliton Clusters in Nonlocal Nonlinear Media},
author ={  D. Buccoliero and  A. S. Desyatnikovand  W. Kr{o}likowski},
journal ={ '' Phys. Rev. Lett. },
volume = {98},
pages = { 053901 },
year = {2007}
}

@article{ Fleischhauer2000,
title ={Dark-State Polaritons in Electromagnetically Induced Transparency},
author ={  M. Fleischhauer and M. D. Lukin and },
journal ={ '' Phys. Rev. Lett. },
volume = {84},
pages = { 5094--5097 },
year = {2000}
}

@article{ Liu2001,
title ={Observation of coherent optical information storage in an atomic medium using halted light pulses},
author ={  C. Liu and  Z. Duttonand  C. H. Behroozi},
journal ={ '' Nature },
volume = {409},
pages = { 490--493 },
year = {2001}
}

@article{ Phillips2001,
title ={Storage of Light in Atomic Vapor},
author ={  D. F. Phillips and  A. Fleischhauerand  A. Mairand  R. L. Walsworth},
journal ={ '' Phys. Rev. Lett. },
volume = {86},
pages = { 783--786 },
year = {2001}
}

@article{ Davidson,
title ={Storing Images in Warm Atomic Vapor},
author ={  M. Shuker and  O. Firstenbergand  R. Pugatchand  A. Ron},
journal ={ '' Phys. Rev. Lett. },
volume = {100},
pages = { 223601 },
year = {2008}
}

@article{ Novikova2012,
title ={Electromagnetically induced transparency-based slow and stored light in warm atoms},
author ={  I. Novikova and  R. L.Walsworth},
journal ={ '' Laser \& Photon. Rev. },
volume = {6},
pages = { 333--353 },
year = {2012}
}

@article{ Chen2013,
title ={Coherent Optical Memory with High Storage Efficiency and Large Fractional Delay},
author ={  Y.-H. Chen and  M.-J. Leeand  I-C. Wangand  S. Duand  Y.-F. Chenand  Y.-C. Chen},
journal ={ '' Phys. Rev. Lett. },
volume = {110},
pages = { 083601 },
year = {2013}
}

@article{ Maxwell2013,
title ={Storage and Control of Optical Photons Using Rydberg Polaritons},
author ={  D. Maxwell and  D. J. Szwerand  D. Paredes-Baratoand  H. Buscheand  J. D. Pritchardand  A. Gauguetand  K. J. Weatherilland  M. P. A. Jones},
journal ={ '' Phys. Rev. Lett. },
volume = {110},
pages = { 103001 },
year = {2013}
}

@article{ Dudin2013,
title ={Light storage on the time scale of a minute},
author ={  Y. O. Dudin and  L. Li},
journal ={ '' Phys. Rev. A },
volume = {87},
pages = { 031801},
year = {R}
}

@article{ Heinze2013,
title ={Stopped Light and Image Storage by Electromagnetically Induced Transparency Up to the Regime of One Minute},
author ={  G. Heinze and  C. Hubrich},
journal ={ '' Phys. Rev. Lett. },
volume = {111},
pages = { 033601 },
year = {2013}
}

@article{ Chen20141,
title ={Ultralow optical solitons and their storage and retrieval in an ultracold ladder-type atomic system},
author ={  Y. Chen and  Z. Bai},
journal ={ " Phys. Rev. A },
volume = {89},
pages = { 023835 },
year = {2014}
}

@article{ Sibalic2016,
title ={Dressed-state electromagnetically induced transparency for light storage in uniform-phase spin waves},
author ={  N.  and  J. M. Kondoand  C. S. Adams},
journal ={ '' Phys. Rev. A },
volume = {94},
pages = { 033840 },
year = {2016}
}

@article{ Hsiao2018,
title ={Highly Efficient Coherent Optical Memory Based on Electromagnetically Induced Transparency},
author ={  Y.-F. Hsiao and  P.-J. Tsaiand  H.-S. Chenand  S.-X. Linand  C.-C. Hungand  C.-H. Leeand  Y.-H. Chenand  Y.-F. Chenand  I.-A. Yu},
journal ={ '' Phys. Rev. Lett. },
volume = {120},
pages = { 183602 },
year = {2018}
}



